Optimal Joint Radar and Communication User Association in Cell-Free mMIMO Systems

The cell-free massive multiple-input multiple-output (CF-mMIMO) systems are crucial for 6G development due to their high spectral efficiency and uniform user-experienced data rates. A key aspect of CF-mMIMO is user association (UA) and optimal cluster formation. Traditional methods focusing solely on communication-related metrics fall short in this context, as sensing is becoming integral to 6G. This study delves into a framework for joint radar and communication (JRC) in CF-mMIMO systems and investigates JRC-based UA techniques. We propose a novel method to optimize UA, enhancing both communication spectral efficiency and sensing accuracy. Existing literature has not explored this dual requirement integration for UA. Our proposed two-step scheme optimizes UA clusters for both communication and sensing. The first step involves selecting access points (APs) based on channel quality, followed by a second step that further refines the selection by choosing APs from the initial group that are also optimal for sensing. We utilize the signal-clutter plus noise ratio to exclude APs with clutter in front of the user equipment (UE) and the AP view angle, ensuring that radar echoes are received only from the specific UE, not the surrounding clutter. Theoretical analysis and simulations demonstrate that the same APs optimized for communication are not necessarily optimal for sensing, highlighting the need for schemes that incorporate sensing requirements in UA. The results show the effectiveness of the proposed method, showing its potential to improve CF-mMIMO system performance in JRC scenarios.

==> AcronymsListFinal.tex <==
\usepackage{etoolbox}
\makeatletter
\newif\ifAC@uppercase@first%
\def\Aclp#1{\AC@uppercase@firsttrue\aclp{#1}\AC@uppercase@firstfalse}%
\def\AC@aclp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acl{#1}s%
	\fi%
}%
\def\Acp#1{\AC@uppercase@firsttrue\acp{#1}\AC@uppercase@firstfalse}%
\def\AC@acp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@ac{#1}s%
	\fi%
}%
\def\Acfp#1{\AC@uppercase@firsttrue\acfp{#1}\AC@uppercase@firstfalse}%
\def\AC@acfp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acf{#1}s%
	\fi%
}%
\def\Acsp#1{\AC@uppercase@firsttrue\acsp{#1}\AC@uppercase@firstfalse}%
\def\AC@acsp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acs{#1}s%
	\fi%
}%
\edef\AC@uppercase@write{\string\ifAC@uppercase@first\string\expandafter\string\MakeUppercase\string\fi\space}%
\def\AC@acrodef#1[#2]#3{%
	\@bsphack%
	\protected@write\@auxout{}{%
		\string\newacro{#1}[#2]{\AC@uppercase@write #3}%
	}\@esphack%
}%
\def\Acl#1{\AC@uppercase@firsttrue\acl{#1}\AC@uppercase@firstfalse}
\def\Acf#1{\AC@uppercase@firsttrue\acf{#1}\AC@uppercase@firstfalse}
\def\Ac#1{\AC@uppercase@firsttrue\ac{#1}\AC@uppercase@firstfalse}
\def\Acs#1{\AC@uppercase@firsttrue\acs{#1}\AC@uppercase@firstfalse}
\robustify\Aclp
\robustify\Acfp
\robustify\Acp
\robustify\Acsp
\robustify\Acl
\robustify\Acf
\robustify\Ac
\robustify\Acs
\makeatother

\acrodef{3GPP}{3rd Generation Partnership Project}
\acrodef{4-QAM}{4-state quadrature amplitude modulation}
\acrodef{4G}{fourth generation}
\acrodef{5G}{fifth generation}
\acrodef{6G}{sixth generation}
\acrodef{8-PSK}{8-state phase shift keying}
\acrodef{16-QAM}{16-state quadrature amplitude modulation}
\acrodef{32-QAM}{32-state quadrature amplitude modulation}
\acrodef{64-QAM}{64-state quadrature amplitude modulation}
\acrodef{128-QAM}{128-state quadrature amplitude modulation}
\acrodef{ACF}{auto-correlation function}
\acrodef{ACI}{adjacent channel interference}
\acrodef{ACLR}{adjacent channel leakage ratio}
\acrodef{ACPR}{adjacent channel power ratio }
\acrodef{ADC}{analog-to-digital converter}
\acrodef{ADSL}{asymmetric digital subscriber line}
\acrodef{AFH}{adaptive frequency hopping}
\acrodef{AIC}{Akaike information criteria}
\acrodef{AI}{artificial Intelligence}
\acrodef{ALRT}{average likelihood ratio test}
\acrodef{AM}{amplitude modulation}
\acrodef{AOA}{angle-of-arrival}
\acrodef{AOD}{angle-of-departure}
\acrodef{AP}{access point}
\acrodef{APs}{access points}
\acrodef{ARQ}{automatic repeat request}
\acrodef{AR}{auto-regressive}
\acrodef{AWGN}{additive white Gaussian noise}
\acrodef{BER}{bit-error-rate}
\acrodef{BE}{best effort service}
\acrodef{BLER}{block error rate}
\acrodef{BPF}{band pass filter}
\acrodef{BPSK}{binary phase shift keying}
\acrodef{BS}{base station}
\acrodef{BSA}{blind signal analysis}
\acrodef{BT}{bandwidth-time}
\acrodef{BW}{bandwidth}
\acrodef{BWA}{broadband wireless access}
\acrodef{CAD}{computer aided design}
\acrodef{CAF}{cyclic autocorrelation function}
\acrodef{CCDF}{complementary cumulative distribution function}
\acrodef{CCI}{co-channel interference}
\acrodef{CDF}{cumulative distribution function }
\acrodef{CDL}{clustered delay line}
\acrodef{CDMA}{code division multiple access }
\acrodef{CDMA}{code division multiple access}
\acrodef{CDP}{code domain power}
\acrodef{CFC}{channel frequency correlation}
\acrodef{CFR}{channel frequency response}
\acrodef{CINR}{carrier-to-inteference-plus-noise ratio}
\acrodef{CIR}{channel impulse response}
\acrodef{CLT}{central limit theorem}
\acrodef{CMA}{constant modulus algorithm}
\acrodef{CNN}{convolutional neural networks}
\acrodef{CP}{cyclic prefix}
\acrodef{CPI}{coherent processing interval}
\acrodef{CRC}{cyclic redundancy check}
\acrodef{CRLB}{Cram\'er-Rao lower bound}
\acrodef{CR}{cognitive radio}
\acrodef{CSD}{cyclic spectral density}
\acrodef{CSIT}{channel state information at the transmitter}
\acrodef{CSI}{channel state information}
\acrodef{CSMA}{carrier sense multiple accessing}
\acrodef{CTS}{clear to send}
\acrodef{DAB}{digital audio broadcasting}
\acrodef{DAC}{digital-to-analog converter}
\acrodef{DC}{direct current}
\acrodef{DDC}{digital down conversion}
\acrodef{DFE}{decision feedback equalizer}
\acrodef{DFRC}{dual function radar communication}
\acrodef{DFS}{dynamic frequency selection}
\acrodef{DFT-S-OFDM}{DFT-Spread-OFDM}
\acrodef{DFT}{discrete Fourier transform}
\acrodef{DL}{deep learning}
\acrodef{DNN}{deep neural network}
\acrodef{DoF}{degrees of freedom}
\acrodef{DS-CDMA}{direct spread code division multiple access}
\acrodef{DSP}{digital signal processor}
\acrodef{DSSS}{direct-sequence spread-spectrum}
\acrodef{DUC}{digital up conversion}
\acrodef{DUT}{device under test}
\acrodef{DVB-T}{terrestrial digital video broadcasting}
\acrodef{DWT}{discrete wavelet transform}
\acrodef{ED}{energy detection}
\acrodef{EDGE}{enhanced data rates for GSM evolution}
\acrodef{EGC}{equal gain-combining}
\acrodef{EM}{electromagnetic}
\acrodef{eMBB}{enhance mobile broadband}
\acrodef{EVM}{error vector magnitude}
\acrodef{FB}{feature-based}
\acrodef{FCH}{frame control header}
\acrodef{FDD}{frequency division duplexing}
\acrodef{FEC}{forward error correction}
\acrodef{FER}{frame-error-rate}
\acrodef{FFT}{fast Fourier transform}
\acrodef{FHMA}{frequency hopped multiple access}
\acrodef{FHSS}{frequency-hopping spread spectrum}
\acrodef{FH}{frequency hopping}
\acrodef{FMCW}{frequency modulated continuous wave}
\acrodef{FPGA}{field-programmable gate array}
\acrodef{FSK}{frequency shift keying}
\acrodef{G-REM}{generalized radio environment monitoring}
\acrodef{GB}{grant-based}
\acrodef{GFSK}{Gaussian frequency shift keying}
\acrodef{GF}{grant-free}
\acrodef{GLRT}{generalized likelihood ratio test}
\acrodef{GMSK}{Gaussian minimum shift keying}
\acrodef{GNSS}{global navigation satellite system}
\acrodef{GoF}{goodness-of-fit}
\acrodef{GOS}{grade of service}
\acrodef{GPP}{general purpose processor}
\acrodef{GPS}{global positioning system}
\acrodef{GSM}{global system for mobile communications}
\acrodef{HMM}{hidden Markov model}
\acrodef{IM}{index modulation}
\acrodef{ICI}{inter-carrier interference}
\acrodef{IDFT}{inverse discrete Fourier transform}
\acrodef{IDMA}{interleave division multiple access}
\acrodef{IDW}{inverse distance weighting}
\acrodef{IEEE}{institute of electrical and electronics engineers}
\acrodef{IFFT}{inverse fast Fourier transform}
\acrodef{IF}{intermediate frequencies}
\acrodef{IMD}{inter-modulation distortion}
\acrodef{INI}{inter-numerology interference}
\acrodef{IoT}{Internet of Things}
\acrodef{IP}{internet protocol}
\acrodef{I/Q}{in-phase and quadrature-phase}
\acrodef{ISI}{inter-symbol interference}
\acrodef{ITU}{International Telecommunication Union}
\acrodef{IUI}{inter-user interference}
\acrodef{IWI}{inter-waveform interference}
\acrodef{JRC}{joint radar and communication}
\acrodef{K-L}{Kullback-Leibler}
\acrodef{LAN}{local area network}
\acrodef{LCR}{level crossing rate}
\acrodef{LDPC}{low density parity coding}
\acrodef{LDS-MA}{low density spreading multiple access}
\acrodef{LFM}{linear frequency modulation}
\acrodef{LFSR}{linear feedback shift register}
\acrodef{LHS}{left-hand side}
\acrodef{LLR}{log-likelihood ratio}
\acrodef{LMMSE}{linear minimum mean-square error}
\acrodef{LMS}{least-mean-square}
\acrodef{LNA}{low noise amplifier}
\acrodef{LoS}{line-of-sight}
\acrodef{LO}{local oscillator}
\acrodef{LS}{least square}
\acrodef{LSTM}{long short-term memory}
\acrodef{LTE}{long term evolution}
\acrodef{LTE-A}{\ac{LTE}-advanced}
\acrodef{LU}{licensed user}
\acrodef{MACA}{multiple access collision avoidance}
\acrodef{MAC}{medium access control}
\acrodef{MAI}{multiple access interference}
\acrodef{MANET}{Mobile Ad-Hoc Network}
\acrodef{MC-CDMA}{multi-carrier code division multiple access}
\acrodef{MCS}{modulation and coding scheme}
\acrodef{MCD}{measurement capable device}
\acrodef{MDL}{minimum descriptive length}
\acrodef{MI}{mutual information}
\acrodef{MIMO}{multiple-input multiple-output}
\acrodef{MLE}{maximum likelihood estimation}
\acrodef{MLSE}{maximum likelihood sequence estimation}
\acrodef{MMSE}{minimum mean-square error}
\acrodef{mMIMO}{massive multiple-input multiple-output}
\acrodef{mMTC}{massive machine type communication}
\acrodef{mmWave}{millimeter wave}
\acrodef{MPA}{message-passing algorithm}
\acrodef{MPC}{multipath component}
\acrodef{MSE}{mean-squared-error}
\acrodef{MSK}{minimum shift keying}
\acrodef{MS}{mobile station}
\acrodef{MUI}{multi user interference}
\acrodef{NBI}{narrow-band interference}
\acrodef{NBF}{narrow-band filter}
\acrodef{NLoS}{non \ac{LoS}}
\acrodef{NN}{neural networks}
\acrodef{NOMA}{non-orthogonal multiple access}
\acrodef{NR}{new radio}
\acrodef{OFDM-CSMA}{OFDM carrier sense multiple accessing}
\acrodef{OFDM-FDMA}{OFDM frequency division multiple accessing}
\acrodef{OFDM-TDMA}{OFDM time division multiple accessing}
\acrodef{OFDMA}{orthogonal frequency division multiple access}
\acrodef{OFDM}{orthogonal frequency division multiplexing}
\acrodef{OK}{Ordinary Kriging}
\acrodef{OMA}{orthogonal multiple access}
\acrodef{OQPSK}{offset quadrature phase‐shift keying}
\acrodef{OSI}{open systems interconnection reference}
\acrodef{OSR}{oversampling rate}
\acrodef{OTA}{over-the-air}
\acrodef{PA}{power amplifier}
\acrodef{PAPR}{peak-to-average power ratio}
\acrodef{PDF}{probability density function}
\acrodef{PDMA}{pattern division multiple access}
\acrodef{PDP}{power delay profile}
\acrodef{PER}{packet-error-rate}
\acrodef{PHY}{physical layer}
\acrodef{PICR}{peak interference-to-carrier ratio}
\acrodef{PLS}{physical layer security}
\acrodef{PMF}{partial match-filtering}
\acrodef{PMP}{point to multi-point}
\acrodef{PN}{pseudo-noise}
\acrodef{PPP}{Poisson point process}
\acrodef{PRBS}{pseudo-random binary sequence}
\acrodef{PRI}{pulse repetition interval}
\acrodef{PRF}{pulse repetition frequency}
\acrodef{PSD}{power spectral density}
\acrodef{PSK}{phase shift keying}
\acrodef{PTS}{partial transmit sequences}
\acrodef{PU}{primary user}
\acrodef{PUSC}{partially used sub-channeling}
\acrodef{QAM}{quadrature amplitude modulation}
\acrodef{QoS}{quality of service}
\acrodef{QPSK}{quadrature phase shift keying}
\acrodef{RACH}{random access channel}
\acrodef{RAT}{radio access technology}
\acrodef{RA}{reconfigurable antenna}
\acrodef{radar}{radio detection and ranging}
\acrodef{RCS}{radar cross section}
\acrodef{RC}{raised cosine}
\acrodef{REM}{radio environment map}
\acrodef{RF-REM}{radio frequency \ac{REM}}
\acrodef{RHS}{right-hand side}
\acrodef{RIS}{reconfigurable intelligent surface}
\acrodef{RL}{reinforcement learning}
\acrodef{RLS}{recursive least-squares}
\acrodef{RMS}{root mean squared}
\acrodef{ROC}{receiver operating characteristic}
\acrodef{RRC}{root raised cosine}
\acrodef{RS}{Reed-Solomon}
\acrodef{RSM}{range sidelobe modulation}
\acrodef{RSSI}{received signal strength indicator}
\acrodef{RTS}{request to send}
\acrodef{RT}{ray-tracing}
\acrodef{RU}{rental user}
\acrodef{RVC}{reverberation chamber}
\acrodef{Rx}{receiver}
\acrodef{SAW}{surface acoustic wave}
\acrodef{SC-FDE}{single carrier frequency domain equalization}
\acrodef{SC-FDMA}{single carrier frequency division multiple access}
\acrodef{SCMA}{sparse code multiple access}
\acrodef{SCS}{sub-carrier spacing}
\acrodef{SC}{selection combining}
\acrodef{SCF}{spectral correlation function}
\acrodef{SDMA}{space-division multiple access}
\acrodef{SDR}{software defined radio}
\acrodef{SDU}{service data unit}
\acrodef{SER}{symbol error rate}
\acrodef{SIC}{successive interference cancellation}
\acrodef{SINR}{signal-to-interference-plus-noise ratio}
\acrodef{SIR}{signal-to-interference ratio}
\acrodef{SISO}{single-input single-output}
\acrodef{SM}{selected mapping}
\acrodef{SNR}{signal-to-noise ratio}
\acrodef{SS}{subscriber station}
\acrodef{STC}{space time coding}
\acrodef{STDCC}{swept time-delay cross correlation}
\acrodef{STFT}{short time Fourier transform}
\acrodef{SVD}{singular value decomposition}
\acrodef{SU}{secondary user}
\acrodef{TDD}{time division duplexing}
\acrodef{TDL}{tapped delay line}
\acrodef{TDMA}{time division multiple access}
\acrodef{TFA}{time-frequency analysis}
\acrodef{TH}{time hopping}
\acrodef{TP}{transmission point}
\acrodef{TVWS}{television white space}
\acrodef{Tx}{transmitter}
\acrodef{UAV}{unmanned aerial vehicles}
\acrodef{UE}{user equipment}
\acrodef{UEs}{user equipments}
\acrodef{UMTS}{universal mobile telecommunications service}
\acrodef{URLLC}{ultra-reliable, low-latency communication}
\acrodef{USRP}{universal software radio peripheral}
\acrodef{UWB}{ultra wide band}
\acrodef{V2V}{vehicle-to-vehicle}
\acrodef{VANET}{vehicular ad-hoc network}
\acrodef{VCO}{voltage-controlled oscillator}
\acrodef{VNA}{vector network analyzer}
\acrodef{VR}{virtual reality}
\acrodef{VSA}{vector signal analyser}
\acrodef{VSG}{vector signal generator}
\acrodef{WCDMA}{wide band code division multiple access}
\acrodef{Wi-Fi}{wireless fidelity}
\acrodef{WiMAX}{worldwide interoperability for microwave access}
\acrodef{WLAN}{wireless local area network}
\acrodef{WMAN}{wireless metropolitan area network}
\acrodef{WPAN}{wireless personal area network}
\acrodef{WRAN}{wireless regional area network}
\acrodef{WSSUS}{wide-sense stationary uncorrelated scattering}
\acrodef{WSS}{wide-sense stationary}
\acrodef{WT}{wavelet transform}
\acrodef{XPR}{cross polarization power ratio}
\acrodef{ZPSK}{zero-padded phase shift keying}
\acrodef{FDMA}{frequency division multiple accessing}

%%%%% Conflicting Acronyms %%%%%%%%%

\acrodef{ML}{machine learning}
% \acrodef{ML}{maximum likelihood}
% \acrodef{CW}{carrier wave}
\acrodef{CW}{continuous wave}
\acrodef{RF}{radio frequency}

% Added by Musab
\acrodef{DTFT}{discrete-time Fourier transform}
\acrodef{PLL}{phase-locked loop}

% Added for Ch7(new)
\acrodef{OOBE}{out-of-band emission}
\acrodef{FDE}{frequency domain equalization}
\acrodef{ZP}{zero-padding}
\acrodef{AFC}{adaptive frequency correction}
\acrodef{SPNIR}{signal-to-phase-noise-interference-ratio}
\acrodef{AM-AM}{amplitude-to-amplitude}
\acrodef{AM-PM}{amplitude-to-phase}
\acrodef{TDM}{time division multiplexing}
\acrodef{NTN}{non-terrestrial network}
\acrodef{ISAC}{integrated sensing and communication}
\acrodef{TN}{terrestrial network}
\acrodef{UAV}{unmanned aerial vehicle}
\acrodef{OCDM}{orthogonal chirp division multiplexing}
\acrodef{OTFS}{orthogonal time frequency space}
\acrodef{SC}{single carrier}
\acrodef{HAPS}{high-altitude platform station}
\acrodef{RAN}{radio access network}
\acrodef{LEO}{low earth orbit}
\acrodef{MEO}{medium earth orbit}
\acrodef{GEO}{geosynchronous equatorial orbit}
\acrodef{PRI}{pulse repetition interval}
\acrodef{OTAC}{Over-the-Air Computation}
\acrodef{JVC-UA}{joint virtual cluster formation and user association}
\acrodef{SOP}{state of polarization}
\acrodef{THz}{terahertz}
\acrodef{RCC}{radar communication coexistence}
\acrodef{XPD}{cross polarization discrimination}
\acrodef{DP}{dual polarized}
\acrodef{RnC}{radar and communication}
\acrodef{SCM}{spatial channel model}
\acrodef{CPU}{central processing unit}
\acrodef{CF-mMIMO}{cell-free mMIMO}
\acrodef{LSFC}{large-scale fading coefficient}
\acrodef{UL}{uplink}
\acrodef{DL}{downlink}
\acrodef{MR}{maximum ratio}
\acrodef{SE}{spectral efficiency}
\acrodef{ES}{exhaustive search}
\acrodef{NP}{non-deterministic Polynomial time}
\acrodef{SCNR}{signal-clutter plus noise power ratio}
\acrodef{PPP}{Poisson point process}
\acrodef{RV}{Random variable}
\acrodef{$P_D$}{Probability of detection}
\acrodef{$P_{dc}$}{radar detection coverage probability}
\acrodef{RMSE}{root mean squared error}
\acrodef{UA}{user association}

